Train High, Ship Low: Efficient LoRA Synchronization for Distributed On-Policy Post-Training

Transmitting LoRA adapters to rollout workers can bottleneck distributed on-policy post-training over bandwidth-constrained networks. Lowering the training rank may limit the capacity a workload needs, while adaptive optimizer updates are difficult to compress. Rollout workers can instead reconstruct updates from gradients by maintaining replicated optimizer states. We introduce HiLo, a compressor-agnostic framework that replaces parameter transmission with compressed gradient dissemination and local optimizer replay. By applying the same decoded gradients, the learner and workers maintain consistent policy states at the same version under reproducible execution. We further develop Spar, a budget-aware gradient compressor that combines spectral truncation, adaptive rank allocation and error feedback to decouple training rank from communication cost. Experiments across on-policy distillation and reward-guided post-training show that HiLo with Spar maintains learning quality close to full synchronization while transmitting as little as 1.6% of the adapter bytes, and accelerates end-to-end updates by up to $2.2\times$ under bandwidth constraints.

==> figures/protocol_tikz.tex <==
\usetikzlibrary{shadows}
\begin{tikzpicture}[
 font=\small, >={Stealth[length=2.1mm,width=1.65mm]},
 flow/.style={->,draw=black!85,line width=.65pt},
 region/.style={draw=#1,line width=.65pt,rounded corners=4pt},
 label/.style={font=\scriptsize,align=center,inner sep=2pt},
 title/.style={font=\small\bfseries,inner sep=0pt},
 block/.style={drop shadow={shadow xshift=1.2pt,shadow yshift=-1.4pt,fill=black,opacity=.24},draw=black!80,line width=.6pt,fill=gray!6,rounded corners=3pt,
 minimum width=16mm,minimum height=9mm,align=center,inner sep=3pt},
 op/.style={drop shadow={shadow xshift=1.2pt,shadow yshift=-1.4pt,fill=black,opacity=.24},draw=black!85,line width=.6pt,trapezium,trapezium left angle=75,
 trapezium right angle=75,shape border rotate=90,fill=#1,
 minimum width=9mm,minimum height=10mm,inner sep=2pt,align=center},
]
\definecolor{tensorblue}{HTML}{668D9D}
\definecolor{tensorred}{HTML}{C88F93}
\definecolor{modulegreen}{HTML}{79A48A}
\definecolor{sectionred}{HTML}{365563}
\definecolor{sectionblue}{HTML}{3D7187}
\definecolor{sectiongreen}{HTML}{5C7E70}
\definecolor{deepblue}{HTML}{345E79}
\definecolor{tensorteal}{HTML}{79A79C}
\definecolor{rollgold}{HTML}{E2D29E}

\draw[region=sectionred] (0.0,3.65) rectangle (12.75,6.95);
\draw[fill=white,draw=sectiongreen!40,rounded corners=4pt,line width=.65pt]
 (.20,-.25) rectangle (12.95,3.22);
\draw[fill=white,draw=sectiongreen!65,rounded corners=4pt,line width=.7pt]
 (.10,-.15) rectangle (12.85,3.32);
\draw[region=sectiongreen,fill=white] (0.0,-0.05) rectangle (12.75,3.42);
\node[title,anchor=west] at (0.2,6.68) {Learner};
\node[title,anchor=west] at (1.25,3.15) {Rollout workers};

\newcommand{\relogradstack}[4]{%
 \ifnum#3=1\relax\colorlet{tensorfill}{tensorteal}\else\colorlet{tensorfill}{tensorblue}\fi
 \foreach \layer in {2,1,0}{
  \pgfmathsetmacro{\depthx}{.07*\layer}
  \pgfmathsetmacro{\depthy}{.16*\layer}
  \pgfmathtruncatemacro{\strength}{100-20*\layer}
  \colorlet{layerfill}{tensorfill!\strength!white}
  \filldraw[drop shadow={shadow xshift=1.2pt,shadow yshift=-1.4pt,fill=black,opacity=.24},fill=layerfill!7,draw=layerfill!75!black,line width=.65pt,rounded corners=1pt]
   (#1-.065+\depthx,#2+.13+\depthy) rectangle (#1+1.265+\depthx,#2+1.17+\depthy);
  \foreach \kind in {0,1}{
   \ifnum\kind=0\relax
    \pgfmathsetmacro{\bx}{#1+\depthx}
    \pgfmathsetmacro{\by}{#2+.25+\depthy}
    \def\ww{.32}\def\hh{.80}\def\nr{5}\def\nc{2}
   \else
    \pgfmathsetmacro{\bx}{#1+.40+\depthx}
    \pgfmathsetmacro{\by}{#2+.49+\depthy}
    \def\ww{.80}\def\hh{.32}\def\nr{2}\def\nc{5}
   \fi
   \foreach \row in {1,...,\nr}{
    \foreach \col in {1,...,\nc}{
     \pgfmathtruncatemacro{\shade}{28+11*mod(\row*3+\col*2+\row*\col,6)}
     \pgfmathsetmacro{\cellx}{\bx+(\col-1)*\ww/\nc}
     \pgfmathsetmacro{\celly}{\by+(\row-1)*\hh/\nr}
     \pgfmathsetmacro{\cellw}{\ww/\nc}
     \pgfmathsetmacro{\cellh}{\hh/\nr}
     \filldraw[fill=layerfill!\shade!white,draw=white,line width=.18pt]
      (\cellx,\celly) rectangle ++(\cellw,\cellh);
    }
   }
   \draw[layerfill!65!black,line width=.55pt]
    (\bx,\by) rectangle ++(\ww,\hh);
  }
 }
 \node[label,inner sep=1pt] at (#1+.60,#2-.10) {#4};
}
\node[minimum width=14mm,minimum height=7mm,inner sep=0pt] (g) at (0.8,4.48) {};
\relogradstack{.20}{4.03}{0}{}
\node[label,font=\fontsize{6.3}{7.2}\selectfont\bfseries,anchor=north] at (0.8,6.00) {Gradient $\vec g_t$};
\node[circle,draw=black,fill=white,inner sep=1pt,line width=.7pt] (plus) at (2.2,4.8) {$+$};
\node[op=deepblue,text=white,shape border rotate=270] (enc) at (3.45,4.8) {$E_{\mathcal B}$};
\node[label,font=\fontsize{6.3}{7.2}\selectfont\bfseries,anchor=north] at (3.45,5.78) {Compressor};
\node[label] at (3.45,4.04) {Pluggable backend};
\draw[flow] (1.58,4.8) -- (plus.west);
\draw[flow] (plus) -- node[label,above] {$\vec h_t$} (enc);
\begin{scope}[shift={(5,4.8)},scale=.8,shift={(-5,-4.8)}]
\node[minimum width=10mm,minimum height=7mm,inner sep=0pt]
 (payload) at (5.0,4.8) {};
\filldraw[fill=tensorblue!40,draw=tensorblue!65!black,line width=.5pt]
 (4.5,5.15) -- (4.65,5.27) -- (5.65,5.27) -- (5.5,5.15) -- cycle;
\filldraw[fill=tensorblue!85,draw=tensorblue!65!black,line width=.5pt]
 (5.5,4.45) -- (5.65,4.57) -- (5.65,5.27) -- (5.5,5.15) -- cycle;
\filldraw[fill=tensorblue!75,draw=tensorblue!65!black,line width=.6pt]
 (4.5,4.45) rectangle (5.5,5.15);
\end{scope}
\node[text=white] at (5.0,4.8) {$z_t$};
\node[label,font=\fontsize{6.3}{7.2}\selectfont\bfseries,anchor=north] at (5.0,5.78) {Compressed\\message};

\draw[flow] (enc.east) -- (payload.west);

\node[op=deepblue,text=white] (dl) at (6.7,4.8) {$D$};
\draw[flow] (5.56,4.8) -- (dl.west);

\node[block,fill=modulegreen,minimum width=10mm,minimum height=10mm] (ol) at (10.12,4.8) {$\Phi_{\mathcal O}$};
\node[label,font=\fontsize{6.3}{7.2}\selectfont\bfseries,anchor=north] at (10.12,5.78) {Optimizer step};

\draw[flow] (dl.east) -- (7.72,4.8);
\draw[flow] (9.20,4.8) -- (ol.west);

\foreach \base in {4.8,2.05}{
 \relogradstack{7.83}{\base-.77}{1}{$\widetilde{\vec g}_t$}
}

\foreach \base in {4.8,2.05}{
 \foreach \lefty in {-.32,0,.32}{
  \foreach \righty in {-.46,-.15,.15,.46}{
   \draw[tensorred!65!black,line width=.35pt,opacity=.40]
    (11.255,\base+\lefty) -- (11.745,\base+\righty);
   \draw[tensorred!65!black,line width=.35pt,opacity=.40]
    (11.745,\base+\righty) -- (12.235,\base+\lefty);
  }
 }
 \foreach \x in {11.255,12.235}{
  \foreach \y in {-.32,0,.32}{
   \filldraw[fill=tensorred!30,draw=tensorred!65!black,line width=.55pt]
    (\x,\base+\y) circle (.085);
  }
 }
 \foreach \y in {-.46,-.15,.15,.46}{
  \filldraw[fill=tensorred!60,draw=tensorred!65!black,line width=.55pt]
   (11.745,\base+\y) circle (.085);
 }
}
\node[label,font=\fontsize{6.3}{7.2}\selectfont\bfseries,anchor=north] at (11.745,5.78) {Updated policy};
\draw[flow] (ol.east) -- (11.095,4.8);
\node[label] at (11.745,3.93) {$(\vec\theta_{t+1},s_{t+1})$};
\fill[black!85] (8.85,5.52) circle (1pt);
\draw[flow] (8.85,5.52) -- (8.85,6.14) -- (2.2,6.14) -- (plus.north);
\node[label,font=\fontsize{6.3}{7.2}\selectfont\bfseries,anchor=north] at (6.7,5.78) {Decode};
\node[label,draw=black,fill=gray!6,rounded corners=3pt,line width=.6pt,inner xsep=6pt,inner ysep=4pt] at (4.8,6.14)
 {Error feedback: $\vec e_{t+1}=\vec h_t-\widetilde{\vec g}_t$};

\draw[flow,preaction={draw=white,line width=3pt}] (payload.south) -- (5.0,3.48) -- (5.0,3.48) -- (5.0,2.05) -- (5.97,2.05);
\node[label,draw=black,fill=gray!6,rounded corners=3pt,line width=.6pt,inner xsep=6pt,inner ysep=4pt,font=\fontsize{6.3}{7.2}\selectfont\bfseries] at (5.0,3.48) {Broadcast $(t,z_t)$};
\node[op=deepblue,text=white] (dw) at (6.7,2.05) {$D$};
\node[label,font=\fontsize{6.3}{7.2}\selectfont\bfseries] at (6.7,2.9) {Decode};
\node[block,fill=modulegreen,minimum width=10mm,minimum height=10mm] (ow) at (10.12,2.05) {$\Phi_{\mathcal O}$};
\node[label,font=\fontsize{6.3}{7.2}\selectfont\bfseries] at (10.12,2.9) {Optimizer replay};
\draw[flow] (dw.east) -- (7.72,2.05);
\draw[flow] (9.20,2.05) -- (ow.west);
\node[label,font=\fontsize{6.3}{7.2}\selectfont\bfseries] at (11.745,2.9) {Local policy};
\draw[flow] (ow.east) -- (11.095,2.05);
\node[block,fill=rollgold,minimum width=24mm,minimum height=7mm] (roll) at (9.55,0.65)
 {Rollout engine};
\draw[flow] (11.745,1.47) -- (11.745,0.65) -- (roll.east);
\draw[flow] (roll.west) -- (0.80,0.65) -- (0.80,4.16);
\draw[fill=gray!6,draw=black!55,rounded corners=3pt,line width=.6pt]
 (1.4,.10) rectangle (5.7,1.77);
\node[label,font=\fontsize{6.3}{7.2}\selectfont\bfseries] at (3.55,1.56)
 {On-policy trajectories};
\foreach \yy/\trajindex/\col in {1.23/1/tensorblue,.84/2/sectiongreen,.45/3/tensorred}{
 \foreach \xx in {1.95,2.52,3.09,3.66}{
  \draw[->,draw=\col!75!black,line width=.5pt,>={Stealth[length=1mm,width=.8mm]}]
   (\xx+.09,\yy)--(\xx+.48,\yy);
 }
 \foreach \xx in {1.95,2.52,3.09,3.66,4.23}{
  \filldraw[fill=\col!25,draw=\col!75!black,line width=.45pt]
   (\xx,\yy) circle (.08);
 }
 \draw[->,draw=\col!75!black,line width=.5pt,>={Stealth[length=1mm,width=.8mm]}]
  (4.32,\yy)--(4.55,\yy);
 \node[label,text=\col!75!black,inner sep=0pt] at (4.73,\yy) {$\cdots$};
 \draw[->,draw=\col!75!black,line width=.5pt,>={Stealth[length=1mm,width=.8mm]}]
  (4.92,\yy)--(5.15,\yy);
 \node[label,text=\col!75!black,inner sep=0pt] at (5.37,\yy) {$\tau_{\trajindex}$};
}
\path (0.0,-0.27) -- (12.75,-0.27);
\end{tikzpicture}


==> figures/spar_tikz.tex <==
\usetikzlibrary{shadows}
\begin{tikzpicture}[
 font=\scriptsize,>={Stealth[length=1.5mm,width=1.1mm]},
 arr/.style={->,draw=black!85,line width=.65pt},
 lab/.style={font=\fontsize{6.3}{7.2}\selectfont,align=center,inner sep=2pt},
 head/.style={lab,font=\fontsize{6.5}{7.5}\selectfont\bfseries},
 op/.style={drop shadow={shadow xshift=1.2pt,shadow yshift=-1.4pt,fill=black,opacity=.24},draw=black!85,fill=spnavy,text=white,trapezium,trapezium left angle=75,
 trapezium right angle=75,shape border rotate=270,minimum width=8mm,
 minimum height=8mm,inner sep=1pt},
]
\definecolor{spblue}{HTML}{668D9D}
\definecolor{spgreen}{HTML}{79A48A}
\definecolor{spred}{HTML}{98757F}
\definecolor{spnavy}{HTML}{345E79}
\definecolor{spteal}{HTML}{79A79C}
\draw[draw=spblue!90!black,rounded corners=3pt,line width=.65pt]
 (0,4.1) rectangle (6,6);
\draw[draw=spgreen,rounded corners=3pt,line width=.65pt]
 (0,2.05) rectangle (6,3.95);
\draw[draw=spred,rounded corners=3pt,line width=.65pt]
 (0,0) rectangle (6,1.9);
\node[head,anchor=west] at (.12,5.77) {1. Extract spectra};
\foreach \layer in {2,1,0}{
 \pgfmathsetmacro{\xx}{.59+.055*\layer}
 \pgfmathsetmacro{\yy}{4.55+.055*\layer}
 \filldraw[drop shadow={shadow xshift=.8pt,shadow yshift=-.9pt,fill=black,opacity=.20},fill=spblue!12,draw=spblue!65!black,line width=.4pt]
  (\xx,\yy) rectangle ++(.28,.70);
 \foreach \row in {0,...,4}{
  \foreach \col in {0,1}{
   \pgfmathtruncatemacro{\shade}{40+10*mod(\row+2*\col,4)}
   \filldraw[fill=spblue!\shade!white,draw=white,line width=.15pt]
    (\xx+.14*\col,\yy+.14*\row) rectangle ++(.14,.14);
  }
 }
 \draw[spblue!65!black,line width=.4pt] (\xx,\yy) rectangle ++(.28,.70);
}
\node[lab] at (.75,4.3) {$H_j\!\in\!\mathbb{R}^{a_j\times b_j}$};
\draw[arr] (1.13,4.97) -- (2.12,4.97);
\draw[drop shadow={shadow xshift=1.2pt,shadow yshift=-1.4pt,fill=black,opacity=.24},fill=spteal,line width=.6pt] (2.25,4.63) rectangle (2.93,5.31);
\foreach \row in {0,1}{
 \foreach \col in {0,1}{
  \pgfmathtruncatemacro{\shade}{65+10*mod(\row+\col,2)}
  \filldraw[fill=spteal!\shade!white,draw=white,line width=.35pt]
   (2.25+.34*\col,4.63+.34*\row) rectangle ++(.34,.34);
 }
}
\draw[spteal!60!black,line width=.6pt] (2.25,4.63) rectangle (2.93,5.31);
\node[lab] at (2.59,4.3) {$K_j=H_j^\top H_j$};
\draw[arr] (3.08,4.97) -- (4.12,4.97);
\node[op] (evd) at (4.72,4.97) {EVD};
\node[lab] at (4.72,4.3) {Eigenpairs};
\draw[arr] (evd.east) -- (5.78,4.97) -- (5.78,4.025) -- (.25,4.025) -- (.25,2.88) -- (.50,2.88);

\node[head,anchor=west] at (.4,3.71) {2. Allocate the byte budget $\mathcal B$};
\foreach \base in {.60,1.32,2.04}{
 \foreach \idx/\height in {0/.57,1/.34,2/.17,3/.08}{
  \pgfmathsetmacro{\blend}{15+20*\base}
  \fill[spblue!\blend!spteal] (\base+\idx*.13,2.56) rectangle ++(.095,\height);
 }
}
\node[lab] at (1.58,3.36) {Spectra $\sigma_{j,\ell}^2$};
\node[lab] at (1.58,2.29) {$c_j=q(a_j+b_j)$ bytes};
\draw[arr] (2.70,2.88) -- (3.24,2.88);
\node[draw=black,fill=gray!6,rounded corners=2pt,align=center,
 font=\fontsize{6.3}{7.2}\selectfont,inner sep=4pt] (alloc) at (4.42,2.88)
 {Greedy allocation\\sort by $\sigma_{j,\ell}^2/c_j$};
\node[lab] at (4.42,2.29) {$\sum_j c_jk_j\leq\mathcal B$};
\draw[arr] (alloc.east) -- (5.78,2.88) -- (5.78,1.975) -- (.25,1.975) -- (.25,.92) -- (.50,.92);

\node[head,anchor=west] at (.4,1.66) {3. Pack low-rank factors};
\foreach \base/\keep in {.60/2,1.32/1,2.04/0}{
 \foreach \idx/\height in {0/.53,1/.32,2/.16,3/.08}{
  \ifnum\idx<\keep\relax\def\barcolor{spgreen}\else\def\barcolor{black!12}\fi
  \fill[\barcolor] (\base+\idx*.13,.65) rectangle ++(.095,\height);
 }
 \node[lab] at (\base+.22,.36) {$\keep$};
}
\node[lab] at (1.58,1.41) {Ranks $k_j$};
\draw[arr] (2.70,.92) -- (3.12,.92);
\node[op] (pack) at (3.72,.92) {Packing};
\draw[arr] (pack.east) -- (4.52,.92);
\foreach \layer in {2,1,0}{
 \pgfmathsetmacro{\xx}{-.03*\layer}
 \pgfmathsetmacro{\yy}{-.05*\layer}
 \filldraw[fill=spblue!85,draw=spblue!65!black,line width=.35pt]
 (4.65+\xx,.71+\yy) -- ++(.14,0) -- ++(.14,.60) -- ++(-.14,0) -- cycle;
 \filldraw[fill=spteal,draw=spblue!65!black,line width=.35pt]
 (5.04+\xx,.99+\yy) -- ++(.50,0) -- ++(.05,.14) -- ++(-.50,0) -- cycle;
}
\node[lab] at (5.13,.31) {$P_j,\ Q_j$};
\path (0,-.17) -- (6,-.17);
\end{tikzpicture}

